Mutation Analysis for Cyber-Physical Systems: Scalable Solutions and Results in the Space Domain

On-board embedded software developed for spaceflight systems (space software) must adhere to stringent software quality assurance procedures. For example, verification and validation activities are typically performed and assessed by third party organizations. To further minimize the risk of human mistakes, space agencies, such as the European Space Agency (ESA), are looking for automated solutions for the assessment of software testing activities, which play a crucial role in this context. Over the years, mutation analysis has shown to be a promising solution for the automated assessment of test suites; it consists of measuring the quality of a test suite in terms of the percentage of injected faults leading to a test failure. A number of optimization techniques, addressing scalability and accuracy problems, have been proposed to facilitate the industrial adoption of mutation analysis. However, to date, two major problems prevent space agencies from enforcing mutation analysis in space software development. In this paper, we enhance mutation analysis optimization techniques to enable their applicability to embedded software and propose a pipeline that successfully integrates them to address scalability and accuracy issues in this context, as described above. Further, we report on the largest study involving embedded software systems in the mutation analysis literature. Our research is part of a research project funded by ESA ESTEC involving private companies (GomSpace Luxembourg and LuxSpace) in the space sector. These industry partners provided the case studies reported in this paper; they include an on-board software system managing a microsatellite currently on-orbit, a set of libraries used in deployed cubesats, and a mathematical library certified by ESA.

==> tables/operator_categories.tex <==

\begin{table}
\scriptsize
\centering
\label{table:codeoperatorssummary}
\caption{Categories of mutation operators applicable to space software.}
\begin{tabular}{p{1.8cm}|p{5.4cm}}
\toprule
Operator Category & Description\\
\midrule
arithmetic & Includes operators that performs mutations on arithmetic expressions and assignments, usually these mutations replaces an element by an operator $op \in \{+, -, *, /, \%\}$. \\
bitwise & Includes operators that performs bitwise mutations on expressions and assignments, these mutations aims for replacing an element of an expression by an operator $op \in \{|, \&, \wedge, \sim\}$. \\
casts & Includes operators that work by mutating casting expressions.\\
constants & Includes operators that mutate constants in the code. \\
control-flow & Includes operators that modify and alter the execution flow of the running application.\\
coverage & Includes operators that mutate the code in such a way that the static structure of the code (e.g., branches) is likely covered during execution.\\
deletion & Includes operators that mutate the code by deleting statements, operators, constants and variables.  \\
floating points & Includes operators working on floating point comparison (FPC).\\
function calls & Includes operators that mutate function calls and their components (e.g., signature and parameters).\\
logical & Includes operators that performs logical mutations on expressions and assignments; these mutations replace an element of an expression by an operator $op \in \{\&\&, \|, !\}$.\\
variable references & Includes operators mutating different types of variable references in the code (e.g., scalars, arrays and pointers).\\
shift & Includes operators that performs shift mutations on expressions and assignments; usually, these mutations replace an element by an operator $op \in \{<<, <<<, >>, >>>\}$.\\
SQL & Includes operators that modify SQL clauses, SQL \texttt{NULL} operators, and SQL \texttt{WHERE} operators.\\
statements & Includes operators performing syntactical changes at a statement-level granularity.\\
strings & Includes operators that performs mutations on variables of string type.\\
structures & Includes operators that mutate C/C++ structures.\\
higher-order & Includes operators for generating second- and higher-order mutants. These strategies combine first order mutants to simulate more complex faults, motivated by a desire to capture subtle faults~\cite{jia2009higher}. Usually, each operator of this category introduce a strategy on how to combine first order operators to form a higher-order one. For example, the \emph{RMix} operator combines any two randomly selected first order operator to generate a higher-order mutant. \\
system-configuration & Includes operators that perform mutations at a system-configuration level; usually, these mutation operators aim to cause faults concerning the configuration of the system itself.\\
system-level & Includes operators that performs mutations at a system-level; usually, these mutation operators aim to cause faults concerning the integration of system components. \\
ADA expressions & Includes operators that work by modifying expressions in the ADA programming language. \\
ADA operands & Includes operators that perform mutations by replacing operands in ADA expressions (e.g., variables, constants, records, arrays, pointers).\\
ADA tasks & Includes operators that mutate ADA code at the granularity of tasks and aim to trigger problems related to concurrency in the program.\\
\bottomrule
\end{tabular}
\end{table}


==> tables/results_CI_reduced_test_suite.tex <==


\begin{table*}[h]
\centering
\scriptsize
\caption{RQ5. CI definition for \APPR Test Suites.}
\label{table:results:ciDefinition} 
\begin{tabular}{|l|l|llllllllll|}
\hline
          &                           & \multicolumn{2}{c}{\GCSP{}} & \multicolumn{2}{c}{\PARAM{}} & \multicolumn{2}{c}{\UTIL{}} & \multicolumn{2}{c}{\MLFS{}{}} & \multicolumn{2}{c|}{\SAIL{}} \\
\hline
Strategy  & Method                    & \#Mutants    & \textbf{$\delta_{acc}$}    & \#Mutants    & \textbf{$\delta_{acc}$}    & \#Mutants    & \textbf{$\delta_{acc}$}   & \#Mutants  & \textbf{$\delta_{acc}$}  & \#Mutants   & \textbf{$\delta_{acc}$}  \\
\hline
$D_J$   & \multirow{4}{*}{CI 0.1}  & 519.1        & 3.55          & 356.7        & 3.62          & 345.8        & 2.54         & 284.6      & 4.07        &    NA         &     NA        \\
$D_O$    &                           				& 518        & 3.55          & 356.7        & 3.62          & 345.8        & 2.54         & 286.1      & 4.07        &       NA     &     NA        \\
$D_E$ &                           					& 449.5        & 3.75          & 356.7        & 3.62          & 345.8        & 2.51         & 259.1      & 4.33        &   1128.8          & 4.78            \\
$D_C$    &                          					 & 448.7        & 3.75          & 356.7        & 3.62          & 343.3        & 2.57         & 258.5      & 4.27        &    1230.8 &   4.88          \\
\hline
$D_J$   & \multirow{4}{*}{CI 0.09} & 667.7        & 3.95          & 439.5        & 3.78          & 424.2        & 2.34         & 352.8      & 4.72        &     NA        &    NA         \\
$D_O$    &                          					 & 665.7        & 3.93          & 439.5        & 3.78          & 424.2        & 2.34         & 353      & 4.72        &        NA     &       NA      \\
$D_E$ &                           					& 567.2        & 3.14          & 439.5        & 3.78          & 422.3         & 2.14         & 316.5      & 5.19        &  1652.2           & 4.88            \\
$D_C$    &                          					 & 566.3        & 3.14          & 439.5        & 3.78          & 421.3        & 2.12         & 316.6      & 5.19        &   1832.8          &  4.92           \\
\hline
$D_J$   & \multirow{4}{*}{CI 0.08} &885.8        & 1.94          & 558.2        & 3.40          & 535.4        & 2.30         & 450.7        & 3.66        &      NA       &       NA      \\
$D_O$    &                           					& 883.8        & 2.04          & 558.2        & 3.40          & 535.4        & 2.30     & 451      & 3.66        &      NA       &   NA          \\
$D_E$ &                          					 & 735.8        & 3.22          & 558.2        & 3.40          & 531.2        & 2.79         & 392.7      & 4.40        &      NA       &   4.24          \\
$D_C$    &                          					 & 734        & 3.23          & 558.2        & 3.40          & 529.9        & 2.76         & 393.4      & 3.85        &     NA        &     4.30        \\
\hline
$D_J$   & \multirow{4}{*}{CI 0.07} & 1235.4       & 2.42          & 730.3        & 2.33          & 709.5        & 2.76         & 599.9      & 2.61       &      NA       &      NA       \\
$D_O$    &                           					& 1231.5       & 2.53          & 730.3        & 2.33          & 709.5        & 2.76         & 600.8        & 2.61        &      NA       &    NA         \\
$D_E$ &                           					& 993.1       & 1.88          & 730.3        & 2.33          & 704.7        & 2.81         & 511        & 4.11        &       NA      &    NA        \\
$D_C$    &                           					& 990.4       & 1.91          & 730.3        & 2.33          & 702          & 2.81         & 508.7      & 4.12        &    NA         &    NA        \\
\hline
$D_J$   & \multirow{4}{*}{CI 0.06} & 1860.4       & 1.92          & 996.8        & 2.26          & 963          & 2.84         & 859.2      & 2.20        &    NA         &  NA           \\
$D_O$    &                          					 & 1852.5       & 1.98          & 996.8        & 2.26          & 963        & 2.84         & 860      & 2.20        &       NA      &      NA       \\
$D_E$ &                           					& 1416       & 1.68          & 996.8        & 2.26          & 955.8        & 2.85         & 709.7      & 2.39        &      NA       &       NA      \\
$D_C$    &                        					   & 1410.9       & 1.74          & 996.8        & 2.26          & 951.9        & 2.85         & 707.8      & 2.39        &     NA        &   NA          \\
\hline
$D_J$   & \multirow{4}{*}{CI 0.05} & NA           & 1.69          & 1438         & 1.61          & 1392       & 2.58         & 1273.4     & 2.24        &    NA         &       NA      \\
$D_O$    &                         					  & NA           & 1.63          & 1438         & 1.61          & 1392       & 2.58         & 1275.7     & 2.20        &     NA        &      NA       \\
$D_E$ &                          					 & 2197       & 1.22          & 1438         & 1.61          & 1377.3       & 2.54         & 1038.6     & 2.18        &       NA      &       NA      \\
$D_C$    &                        					   & 2187.9       & 1.23          & 1438         & 1.61          & 1370         & 2.48         & 1035.8     & 2.10        &   NA          &     NA       \\
\hline
\end{tabular}
\end{table*}


==> tables/results_prioritize_accuracy.tex <==




\begin{table*}
\tiny
\centering
\caption{RQ6. P-value comparison between test suite reduction approaches.}
\label{table:results:pValComparisonTSredPrior} 
\begin{tabular}{|l|l|lllll|l|lllll|}
\hline
           &          & ALL      &                       &                       &          &      &          & SDL      &                       &                       &                       &       \\
\hline           
Case Study &          & Baseline & $D_J$                  & $D_O$                  & $D_E$     & $D_C$ &          & Baseline & $D_J$                  & $D_O$                  & $D_E$                  & $D_C$  \\
\hline
\GCSP{}   & Baseline &          &                       &                       &          &      & Baseline &          &                       &                       &                       &       \\
           & $D_J$     & 1.47E-04 &                       &                       &          &      & $D_J$     & 1.37E-04 &                       &                       &                       &       \\
           & $D_O$     & 1.40E-04 & 2.50E-01              &                       &          &      & $D_O$     & 1.18E-04 & 7.88E-02              &                       &                       &       \\
           & $D_E$     & 5.18E-05 & 5.15E-05              & 4.81E-05              &          &      & $D_E$     & 5.30E-04 & 4.56E-04              & 3.80E-05              &                       &       \\
           & $D_C$     & 1.17E-04 & 1.16E-04              & 1.10E-04              & 2.93E-02 &      & $D_C$     & 1.08E-04 & 9.55E-05              & 8.21E-05              & 6.71E-02              &       \\
\hline
\UTIL{}    & Baseline &          &                       &                       &          &      & Baseline &          &                       &                       &                       &       \\
           & $D_J$     & 1.27E-04 &                       &                       &          &      & $D_J$     & 1.23E-04 &                       &                       &                       &       \\
           & $D_O$     & 1.20E-04 & 8.31E-01              &                       &          &      & $D_O$     & 1.15E-04 & 8.31E-01              &                       &                       &       \\
           & $D_E$     & 1.20E-04 & 8.38E-03              & 2.05E-03              &          &      & $D_E$     & 1.15E-04 & 8.31E-01              & \multicolumn{1}{r}{1} &                       &       \\
           & $D_C$     & 1.31E-04 & 6.40E-03              & 2.20E-03              & 5.34E-01 &      & $D_C$     & 1.26E-04 & 6.80E-01              & 5.34E-01              & 5.34E-01              &       \\
\hline
\PARAM{}   & Baseline &          &                       &                       &          &      & Baseline &          &                       &                       &                       &       \\
           & $D_J$     & 5.38E-05 &                       &                       &          &      & $D_J$     & 4.96E-05 &                       &                       &                       &       \\
           & $D_O$     & 5.38E-05 & \multicolumn{1}{r}{1} &                       &          &      & $D_O$     & 4.96E-05 & \multicolumn{1}{r}{1} &                       &                       &       \\
           & $D_E$     & 5.38E-05 & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} &          &      & $D_E$     & 4.96E-05 & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} &                       &       \\
           & $D_C$     & 5.38E-05 & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} &    \multicolumn{1}{r}{1}   &      & $D_C$     & 4.96E-05 & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{1} &       \\
\hline
\MLFS{}{}       & Baseline &          &                       &                       &          &      & Baseline &          &                       &                       &                       &       \\
           & $D_J$     & 1.40E-04 &                       &                       &          &      & $D_J$     & 5.30E-05 &                       &                       &                       &       \\
           & $D_O$     & 1.40E-04 & \multicolumn{1}{r}{1} &                       &          &      & $D_O$     & 5.30E-05 & \multicolumn{1}{r}{1} &                       &                       &       \\
           & $D_E$     & 1.36E-04 & 1.20E-04              & 1.20E-04              &          &      & $D_E$     & 5.30E-05 & 1.31E-05              & 1.31E-05              &                       &       \\
           & $D_C$     & 1.48E-04 & 1.31E-04              & 1.31E-04              & 1.61E-02 &      & $D_C$     & 5.30E-05 & 1.31E-05              & 1.31E-05              & \multicolumn{1}{r}{1} &       \\
\hline
\SAIL{}     & Baseline &                     &                       &                  &          &      & Baseline &          &                       &                       &                       &       \\
              	 & $D_J$     &  1.50E-04&                       &                      &                   &      & $D_J$     &   1.45E-04&                       &                       &                       &       \\
           		& $D_O$     &   1.52E-04&     1.28E-01  &                       &                   &      & $D_O$     &  1.43E-04&4.61E-01&&&       \\
           		& $D_E$     &   1.52E-04&     1.49E-04   &    1.52E-04   &                   &      & $D_E$     &  1.48E-04&1.45E-04&1.43E-04&&       \\
           		& $D_C$     &   1.35E-04&      1.32E-04   &    1.34E-04  &    2.42E-02 &      & $D_C$     &  1.28E-04&1.25E-04&1.23E-04&1.71E-04&      \\
\hline           
\end{tabular}
\end{table*}



==> tables/results_reductionFixed.tex <==

\begin{table}[h]
\caption{RQ3. Accuracy of Mutation Sampling with a Predefined Number of Sampled Mutants.}
\label{table:results:fixedNumberOfMutants} 
\tiny
\begin{tabular}{|
p{15mm}p{15mm}
p{1mm}
p{1.5mm}p{1.5mm}
|}
\hline
\textbf{Case Study}&\textbf{Sampling type}&\multicolumn{3}{c|}{\textbf{Values of}}\\
&&\multicolumn{3}{c|}{\textbf{2.5\% - 97.5\% quantiles, for $S$ sampled mutants.}}\\ 
\hline
&&S=&\textbf{100}&\textbf{1000}
\\
$\mathit{\SAIL{}}_{S}$&Random
&&0.01&0.02
\\
..
\\
$\mathit{\SAIL{}}_{S}$&Method-based
&&0.01&0.02 
\\
..
\\
\end{tabular}

\end{table}


==> tables/rq4.tex <==
\begin{table}[htb]
\caption{RQ3. 
Accuracy of proportional uniform sampling applied to select SDL mutants only.}
\label{table:results:accuracy:regSamplingSDL} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{5mm}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
     & \multicolumn{2}{c|}{\textbf{\GCSP{}}} & \multicolumn{2}{c|}{\textbf{\PARAM{}}} & \multicolumn{2}{c|}{\textbf{\UTIL{}}} & \multicolumn{2}{c|}{\textbf{\MLFS{}{}}} & \multicolumn{2}{c|}{\textbf{\SAIL{}}} \\
\hline
\textbf{r=} & \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}               \\
\hline           
0.01 & 10 & 34.36    & 8 & 38.18     & 24 & 16.30   & 18 & 20.69 &       \\
0.02 & 19 & 23.83    & 15 & 29.12    & 47 & 13.91   & 35 & 15.34 &       \\
0.03 & 28 & 20.07    & 22 & 23.67    & 71 & 14.72   & 52 & 12.43 &       \\
0.04 & 37 & 19.56    & 30 & 20.87    & 94 & 11.27   & 70 & 11.06 &       \\
0.05 & 46 & 18.11    & 37 & 17.77    & 118 & 9.31    & 87 & 10.15 &       \\
0.06 & 55 & 15.32    & 44 & 21.39    & 141 & 9.31    & 104 & 9.09  &       \\
0.07 & 64 & 15.61    & 52 & 16.28    & 164 & 9.64    & 122 & 9.18  &       \\
0.08 & 73 & 13.81    & 59 & 16.58    & 188 & 6.99    & 139 & 9.57  &       \\
0.09 & 83 & 11.53    & 66 & 16.16    & 211 & 8.20    & 156 & 8.28  &       \\
0.1  & 92 & 13.19    & 74 & 15.07    & 235 & 7.97    & 173 & 9.25  &       \\
0.2  & 183 & 10.32    & 147 & 9.94     & 469 & 5.25    & 346 & 6.64  &       \\
0.3  & 274 & 9.91     & 220 & 9.12     & 703 & \textbf{4.91}    & 519 & 7.13  &       \\
0.4  & 365 & 8.48     & 292 & 8.73     & 937 & \textbf{4.43}    & 692 & 6.06  &       \\
0.5  & 456 & 8.07     & 364 & 7.38     & 1171 & \textbf{3.61}    & 865 & 5.60  &       \\
0.6  & 548 & 7.17     & 438 & 7.28     & 1405 & \textbf{3.50}    & 1038 & 5.25  &       \\
0.7  & 639 & 6.90     & 510 & 5.86     & 1639 & \textbf{3.27}    & 1211 & \textbf{4.91}  &       \\
0.8  & 730 & 6.56     & 582 & 5.79     & 1873 & \textbf{2.80}    & 1384 & \textbf{4.87}  &       \\
0.9  & 821 & 5.86     & 655 & 5.22     & 2107 & \textbf{2.58}    & 1557 & \textbf{4.49}  &   \\
\hline   
\end{tabular}
Note: \#M, number of mutants. Accurate results (i.e., $\delta_{acc} \le 5\%$) are in bold.
\end{table}


\begin{table}[htb]
\caption{RQ3. 
Accuracy of proportional method-based sampling applied to select SDL mutants only.}
\label{table:results:accuracy:funcSamplingSDL} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{5mm}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
     & \multicolumn{2}{c|}{\textbf{\GCSP{}}} & \multicolumn{2}{c|}{\textbf{\PARAM{}}} & \multicolumn{2}{c|}{\textbf{\UTIL{}}} & \multicolumn{2}{c|}{\textbf{\MLFS{}{}}} & \multicolumn{2}{c|}{\textbf{\SAIL{}}} \\
\hline
\textbf{r=} & \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}               \\
\hline
0.01 & NA       			& NA       		& 4 & 28.80   			& 4 & 31.80 &       \\
0.02 & NA       			& 2 & 69.12    & 15 & 28.80   			& 20 & 18.20 &       \\
0.03 & 2 & 34.36    		& 8 & 44.12    & 28 & 18.09   			& 35 & 15.34 &       \\
0.04 & 10 & 34.36    		& 9 & 35.79    & 44 & 15.16   			& 76 & 12.94 &       \\
0.05 & 12 & 26.03    		& 9 & 35.79    & 64 & 14.00   			& 88 & 11.98 &       \\
0.06 & 15 & 21.03    		& 19 & 24.51    & 88 & 10.62  			 & 109 & 9.94  &       \\
0.07 & 19 & 18.57    		& 25 & 21.12    & 108 & 10.33  			 & 132 & 8.35  &       \\
0.08 & 25 & 22.36    		& 42 & 19.12    & 135 & 6.97   			 & 146 & 8.61  &       \\
0.09 & 40 & 14.36   		 & 46 & 19.12    & 155 & 8.19   			 & 161 & 8.88  &       \\
0.1  & 56- 11.15     		& 57 & 15.67    & 174 & 8.41    			& 176 & 8.54  &       \\
0.2  & 169 & 7.45     		& 153 & 10.68    & 438 & 5.97    			& 348 & 7.43  &       \\
0.3  & 268 & 7.12     		& 238 & 9.46     & 706 & \textbf{3.17}    & 528 & 6.18  &       \\
0.4  & 370 & 7.60     		& 307 & 8.25     & 948 & \textbf{2.85}    & 703 & 5.40  &       \\
0.5  & 446 & 6.78     		& 377 & 8.01     & 1171 & \textbf{3.57}    & 872 & 5.53  &       \\
0.6  & 559 & 5.38     		& 460 & 6.76     & 1445 & \textbf{2.86}    & 1053 & 5.05  &       \\
0.7  & 653 & 5.26     		& 534 & 6.37     & 1686 & \textbf{2.67}    & 1225 & \textbf{4.45}  &       \\
0.8  & 726 & 5.43     		& 599 & 5.86     & 1899 & \textbf{2.08}    & 1396 & \textbf{4.30}  &       \\
0.9  & 808 & \textbf{4.47}     & 675 & 5.35     & 2120 & \textbf{2.03}    & 1567 & \textbf{4.07}  &   \\
\hline     
\end{tabular}
Note: \#M, number of mutants. Accurate results (i.e., $\delta_{acc} \le 5\%$) are in bold.
\end{table}


\begin{table}[htb]
\caption{RQ3. 
Accuracy of proportional uniform sampling applied to select SDL+OODL mutants only.}
\label{table:results:accuracy:regSamplingSDLOODL} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{5mm}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
     & \multicolumn{2}{c|}{\textbf{\GCSP{}}} & \multicolumn{2}{c|}{\textbf{\PARAM{}}} & \multicolumn{2}{c|}{\textbf{\UTIL{}}} & \multicolumn{2}{c|}{\textbf{\MLFS{}{}}} & \multicolumn{2}{c|}{\textbf{\SAIL{}}} \\
\hline
\textbf{r=} & \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}               \\
\hline
0.01 & 16 & 28.11    & 14 & 26.26    & 39 & 12.23   & 60 & 12.41 &       \\
0.02 & 31 & 21.46    & 27 & 19.21    & 77 & 12.60   & 120 & 10.70 &       \\
0.03 & 47 & 16.33    & 40 & 16.62    & 115 & 10.54   & 180 & 10.42 &       \\
0.04 & 62 & 13.39    & 53 & 11.62    & 153 & 7.88    & 239 & 10.47 &       \\
0.05 & 78 & 14.52    & 67 & 12.40    & 191 & 6.81    & 299 & 9.34  &       \\
0.06 & 93 & 13.93    & 80 & 11.03    & 229 & 6.53    & 359 & 9.71  &       \\
0.07 & 109 & 13.26    & 92 & 9.98     & 267 & 5.97    & 418 & 9.00  &       \\
0.08 & 124 & 11.78    & 106 & 13.01    & 305 & 6.02    & 478 & 8.48  &       \\
0.09 & 140 & 13.68    & 120 & 8.29     & 343 & 5.78    & 538 & 9.00  &       \\
0.1  & 155 & 11.13    & 133 & 9.72     & 382 & 5.38    & 598 & 8.67  &       \\
0.2  & 310 & 10.34    & 265 & 7.99     & 763 & \textbf{3.58}    & 1195 & 7.99  &       \\
0.3  & 464 & 9.04     & 398 & 6.31     & 1144 & \textbf{3.59}    & 1792 & 7.52  &       \\
0.4  & 619 & 8.03     & 529 & 5.54     & 1525 & \textbf{3.26}    & 2389 & 7.03  &       \\
0.5  & 773 & 7.65     & 659 & 5.45     & 1906 & \textbf{2.97}    & 2986 & 7.11  &       \\
0.6  & 928 & 7.48     & 795 & \textbf{4.53}     & 2287 & \textbf{2.41}    & 3583 & 6.90  &       \\
0.7  & 1083 & 7.08     & 926 & \textbf{4.24}     & 2668 & \textbf{2.31}    & 4180 & 6.76  &       \\
0.8  & 1237 & 6.79     & 1058 & \textbf{3.75}     & 3049 & \textbf{2.10}    & 4777 & 6.70  &       \\
0.9  & 1392 & 6.38     & 1189 & \textbf{3.56}     & 3430 & \textbf{1.97}    & 5374 & 6.50  &      \\
\hline 
\end{tabular}
Note: \#M, number of mutants. Accurate results (i.e., $\delta_{acc} \le 5\%$) are in bold.
\end{table}


\begin{table}[htb]
\caption{RQ3. 
Accuracy of proportional method-based sampling applied to select SDL+OODL mutants.}
\label{table:results:accuracy:funcSamplingSDLOODL} 
\scriptsize
\centering
\begin{tabular}{|
@{\hspace{1pt}}p{5mm}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{7mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
 >{\raggedleft\arraybackslash}p{8mm}@{\hspace{1pt}}|
  >{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
     & \multicolumn{2}{c|}{\textbf{\GCSP{}}} & \multicolumn{2}{c|}{\textbf{\PARAM{}}} & \multicolumn{2}{c|}{\textbf{\UTIL{}}} & \multicolumn{2}{c|}{\textbf{\MLFS{}{}}} & \multicolumn{2}{c|}{\textbf{\SAIL{}}} \\
\hline
\textbf{r=} & \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}& \textbf{\#M}&\textbf{$\delta_{acc}$}               \\
\hline
0.01 & NA 	   	    & NA       & 9 & 28.80   & 59 & 14.81 &       \\
0.02 & 2 & 65.64    & 7 & 40.55    & 34 & 19.98   & 122 & 11.64 &       \\
0.03 & 18 & 17.69    & 14 & 26.26    & 67 & 10.89   & 195 & 11.02 &       \\
0.04 & 23 & 17.81    & 39 & 14.05    & 97 & 9.21    & 249 & 10.00 &       \\
0.05 & 45 & 16.58    & 55 & 11.84    & 132 & 7.59    & 308 & 9.28  &       \\
0.06 & 66 & 12.43    & 77 & 11.36    & 176 & 6.37    & 379 & 8.84  &       \\
0.07 & 86 & 13.49    & 89 & 10.69    & 230 & 7.93    & 436 & 8.69  &       \\
0.08 & 104 & 11.28    & 102 & 10.30    & 272 & 7.86    & 498 & 8.87  &       \\
0.09 & 120 & 10.19    & 120 & 9.95     & 310 & 6.22    & 552 & 8.70  &       \\
0.1  & 138 & 11.21    & 134 & 9.06     & 354 & 6.21    & 609 & 8.10  &       \\
0.2  & 312 & 7.76     & 283 & 7.11     & 776 & \textbf{3.35}    & 1212 & 8.05  &       \\
0.3  & 471 & 6.56     & 416 & 6.57     & 1166 & \textbf{2.95}    & 1812 & 7.44  &       \\
0.4  & 627 & 7.33     & 548 & 5.90     & 1563 & \textbf{2.47}    & 2411 & 6.88  &       \\
0.5  & 771 & 7.25     & 675 & 5.22     & 1935 & \textbf{2.24}    & 2993 & 6.93  &       \\
0.6  & 943 & 6.63     & 826 & \textbf{4.63}     & 2353 & \textbf{2.03}    & 3598 & 6.73  &       \\
0.7  & 1101 & 6.20     & 958 & \textbf{4.11}     & 2753 & \textbf{1.91}    & 4197 & 6.61  &       \\
0.8  & 1238 & 6.01     & 1082 & \textbf{3.92}     & 3098 & \textbf{1.56}    & 4793 & 6.56  &       \\
0.9  & 1389 & 5.67     & 1217 & \textbf{3.64}     & 3481 & \textbf{1.44}    & 5391 & 6.42  &      \\
\hline 
\end{tabular}
\end{table}




\begin{table*}[htb]
\caption{RQ3. Accuracy with uniform fixed-size sampling and uniform FSCI sampling applied to select SDL mutants. }
\label{table:results:accuracy:sampling_sdl} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
}
\hline
\multicolumn{3}{|c|}{\textbf{\GCSP{}}}      & \multicolumn{3}{c|}{\textbf{\PARAM{}}}      & \multicolumn{3}{c|}{\textbf{\UTIL{}}}       & \multicolumn{3}{c|}{\textbf{\MLFS{}{}}}          & \multicolumn{3}{c|}{\textbf{\SAIL{}}}       \\
\hline
\textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method} \\
\hline
100       & 12.36      & FIXED    & 100       & 12.65      & FIXED    & 100       & 9.32       & FIXED    & 100       & 9.20       & FIXED    &           &            &        \\
200       & 9.36       & FIXED    & 200       & 9.65       & FIXED    & 200       & 7.80       & FIXED    & 199       & 11.44      & CI 0.1  &           &            &        \\
300       & 9.53       & FIXED    & 300       & 7.63       & FIXED    & 300       & 6.97       & FIXED    & 200       & 8.46       & FIXED    &           &            &        \\
335       & 8.88       & CI 0.1  & 367       & 7.15       & CI 0.1  & 317       & 6.81       & CI 0.1  & 244       & 9.38       & CI 0.09 &           &            &        \\
400       & 7.36       & FIXED    & 400       & 7.25       & FIXED    & 390       & 5.91       & CI 0.09 & 300       & 7.04       & FIXED    &           &            &        \\
412       & 8.33       & CI 0.09 & 452       & 6.48       & CI 0.09 & 400       & 5.55       & FIXED    & 310       & 8.82       & CI 0.08 &           &            &        \\
500       & 7.57       & FIXED    & 500       & 6.43       & FIXED    & 492       & 5.05       & CI 0.08 & 400       & 6.20       & FIXED    &           &            &        \\
520       & 7.50       & CI 0.08 & 569       & 5.51       & CI 0.08 & 500       & 5.50       & FIXED    & 405       & 8.04       & CI 0.07 &           &            &        \\
600       & 7.53       & FIXED    & 600       & 5.87       & FIXED    & 600       & 5.47       & FIXED    & 500       & 6.41       & FIXED    &           &            &        \\
676       & 7.09       & CI 0.07 & 700       & \textbf{4.98}       & FIXED    & 639       & \textbf{4.42}       & CI 0.07 & 551       & 6.74       & CI 0.06 &           &            &        \\
700       & 6.79       & FIXED    & NA        & NA         & CI 0.07 & 700       & \textbf{4.73}       & FIXED    & 600       & 5.70       & FIXED    &           &            &        \\
800       & 6.11       & FIXED    & NA        & NA         & CI 0.06 & 800       & \textbf{4.42}       & FIXED    & 700       & 6.06       & FIXED    &           &            &        \\
900       & 5.42       & FIXED    & NA        & NA         & CI 0.05 & 865       & \textbf{4.32}       & CI 0.06 & 791       & 5.78       & CI 0.05 &           &            &        \\
NA        & NA         & CI 0.06 &           &            &          & 900       & \textbf{4.25}       & FIXED    & 800       & 5.70       & FIXED    &           &            &        \\
NA        & NA         & CI 0.05 &           &            &          & 1000      & \textbf{4.65}       & FIXED    & 900       & 5.59       & FIXED    &           &            &        \\
          &            &          &           &            &          & 1242      & \textbf{3.73}       & CI 0.05 & 1000      & \textbf{4.80}       & FIXED    &           &            & \\
\hline       
\end{tabular}
\end{table*}



\begin{table*}[htb]
\caption{RQ4. Accuracy with uniform fixed-size / FSCI sampling applied to select SDL+OODL mutants.}
\label{table:results:accuracy:sampling_sdl_oodl} 
\scriptsize
\centering
\begin{tabular}{|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{10mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
p{12mm}@{\hspace{1pt}}|
}
\hline
\multicolumn{3}{|c|}{\textbf{\GCSP{}}}      & \multicolumn{3}{c|}{\textbf{\PARAM{}}}      & \multicolumn{3}{c|}{\textbf{\UTIL{}}}       & \multicolumn{3}{c|}{\textbf{\MLFS{}{}}}          & \multicolumn{3}{c|}{\textbf{\SAIL{}}}       \\
\hline
\textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method}   & \textbf{\#Mutants} & $\delta_{acc}$ & \textbf{Method} \\
\hline
100       & 14.89      & FIXED    & 100       & 12.22      & FIXED    & 100       & 9.80       & FIXED    & 100       & 12.20      & FIXED    &           &            &        \\
200       & 12.39      & FIXED    & 200       & 8.15       & FIXED    & 200       & 5.56       & FIXED    & 173       & 16.35      & CI 0.1  &           &            &        \\
300       & 9.53       & FIXED    & 300       & 6.80       & FIXED    & 300       & 5.64       & FIXED    & 200       & 10.20      & FIXED    &           &            &        \\
330       & 9.75       & CI 0.1  & 361       & 7.36       & CI 0.1  & 323       & 6.20       & CI 0.1  & 213       & 16.53      & CI 0.09 &           &            &        \\
400       & 9.13       & FIXED    & 400       & 6.87       & FIXED    & 397       & 6.42       & CI 0.09 & 267       & 12.27      & CI 0.08 &           &            &        \\
406       & 9.36       & CI 0.09 & 443       & 6.03       & CI 0.09 & 400       & 6.05       & FIXED    & 300       & 9.37       & FIXED    &           &            &        \\
500       & 8.67       & FIXED    & 500       & 5.92       & FIXED    & 500       & 5.11       & FIXED    & 343       & 11.41      & CI 0.07 &           &            &        \\
512       & 8.77       & CI 0.08 & 558       & 5.62       & CI 0.08 & 502       & \textbf{4.97}       & CI 0.08 & 400       & 9.09       & FIXED    &           &            &        \\
600       & 8.95       & FIXED    & 600       & 4.96       & FIXED    & 600       & \textbf{4.63}       & FIXED    & 477       & 9.22       & CI 0.06 &           &            &        \\
664       & 8.45       & CI 0.07 & 700       & 5.35       & FIXED    & 651       & 5.09       & CI 0.07 & 500       & 8.91       & FIXED    &           &            &        \\
700       & 8.43       & FIXED    & 725       & 5.11       & CI 0.07 & 700       & \textbf{4.02}       & FIXED    & 600       & 8.45       & FIXED    &           &            &        \\
800       & 7.36       & FIXED    & 800       & \textbf{4.74}       & FIXED    & 800       & \textbf{3.42}       & FIXED    & 680       & 8.90       & CI 0.05 &           &            &        \\
900       & 7.48       & FIXED    & 900       & \textbf{4.12}       & FIXED    & 879       & \textbf{4.33}       & CI 0.06 & 700       & 8.20       & FIXED    &           &            &        \\
900       & 7.76       & CI 0.06 & 983       & \textbf{4.17}       & CI 0.06 & 900       & \textbf{3.80}       & FIXED    & 800       & 7.95       & FIXED    &           &            &        \\
1000      & 7.27       & FIXED    & 1000      & \textbf{4.13}       & FIXED    & 1000      & \textbf{3.70}       & FIXED    & 900       & 8.04       & FIXED    &           &            &        \\
1295      & 6.71       & CI 0.05 & NA        & NA         & CI 0.05 & 1261      & \textbf{3.84}       & CI 0.05 & 1000      & 8.11       & FIXED    &           &            &       \\
\hline       
\end{tabular}
\end{table*}



